Learning Image Representations by Completing Damaged Jigsaw Puzzles

In this paper, we explore methods of complicating self-supervised tasks for representation learning. That is, we do severe damage to data and encourage a network to recover them. First, we complicate each of three powerful self-supervised task candidates: jigsaw puzzle, inpainting, and colorization. In addition, we introduce a novel complicated self-supervised task called "Completing damaged jigsaw puzzles" which is puzzles with one piece missing and the other pieces without color. We train a convolutional neural network not only to solve the puzzles, but also generate the missing content and colorize the puzzles. The recovery of the aforementioned damage pushes the network to obtain robust and general-purpose representations. We demonstrate that complicating the self-supervised tasks improves their original versions and that our final task learns more robust and transferable representations compared to the previous methods, as well as the simple combination of our candidate tasks. Our approach achieves state-of-the-art performance in transfer learning on PASCAL classification and semantic segmentation.

==> tables.tex <==
%% Tabel 5, Element-wise operation
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c c c c}
\hline
     Extra ConvBlock & {\bf SUM} &  MAX &PRODUCT \\
\hline
    {\bf w 3x3Conv} & {\bf 78.8 (76.4)}     & 78.9 (76.2)   & 78.3\\
    w/o 3x3Conv     & 78.2                  & 77.8          & -   \\
\hline
\end{tabular}
}
% \bigskip
\smallskip
\caption{{\bf Effects of Extra ConvBlock and Combining Methods} Metric: detection mAP(\%) on VOC07 \textit{test}. ( \ ): detection results of PASCAL VOC12 \textit{test}.}
% \label{tab:table5}
\label{table:ele_op}
\end{table} 

%%% Table 6, Ablation study
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c |c c c |c c c c |c}
                    & SSD     &           &           &           &           &           &           & {\bf StairNet}\\
\hline
    \{2, 3\}        &         &\checkmark &\checkmark &           &\checkmark &\checkmark &\checkmark &\checkmark \\
    deconv          &         &           &\checkmark &\checkmark &           &\checkmark &\checkmark &\checkmark\\
    3x3 conv        &         &           &           &\checkmark &\checkmark &           &\checkmark &\checkmark\\
    unified         &         &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &           & \checkmark \\
\hline
    \{1.6, 2, 3\}   &         &           &           &\checkmark &           &           &\\
    bilinear        &         &           &           &           &\checkmark &           &\\
    ResBlock        &         &           &           &           &           &\checkmark &\\
    multi           &         &           &           &           &           &           &\checkmark &\\
\hline
    VOC 2007 mAP    & 77.2    & 77.4      & 78.2      & 78.9      & 78.5      & 78.6      & 78.9      & {\bf 78.8}\\
\end{tabular}
}
% \bigskip
\smallskip
\caption{{\bf Ablation Experiments on StairNet.} Each component of the first row corresponds to each component of the second row in an one-to-one manner. {\bf \{2,3\} and \{1.6, 2, 3\}} indicates the aspect ratio of the default boxes. {\bf deconv and bilinear} indicates the upsampling method in the feature combining module. {\bf 3x3 conv and ResBlock} indicates the extra layers in the feature combining module. {\bf unified and multi} indicates whether the prediction layer shares the weight or not.}
% \label{tab:table6}
\label{table:ablation}
\end{table} 


%%% Table 1, results on VOC 2007
\begin{table*}
\resizebox{\textwidth}{!}{\begin{tabular}{c| c| c| c | c c c c c c c c c c c c c c c c c c c c c }
\hline
Method & data & network & map & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & horse & mbike & persn & plant & sheep & sofa & train & tv\\
\hline
HyperNet \cite{kong2016hypernet}            & 07+12   & VGGNet       & 76.3
    & 77.4 & 83.3 & 75.0 & 69.1 & 62.4 
    & 83.1 & 87.4 & 87.4 & 57.1 & 79.8 
    & 71.4 & 85.1 & 85.1 & 80.0 & 79.1 
    & 51.2 & 79.1 & 75.7 & 80.9 & 76.5 \\
    
Fr R-CNN \cite{ren2015faster}           & 07+12   & ResNet-101   & 76.4 
    & 79.8 & 80.7 & 76.2 & 68.3 & 55.9 
    & 85.1 & 85.3 & 89.8 & 56.7 & 87.8 
    & 69.4 & 88.3 & 88.9 & 80.9 & 78.4 
    & 41.7 & 78.6 & 79.8 & 85.3 & 72.0 \\

ION \cite{bell2016inside}                   & 07+12+S & VGGNet       & 76.5 
    & 79.2 & 79.2 & 77.4 & 69.8 & 55.7 
    & 85.2 & 84.2 & 89.8 & 57.5 & 78.5 
    & 73.8 & 87.8 & 85.9 & 81.3 & 75.3 
    & 49.7 & 76.9 & 74.6 & 85.2 & 82.1 \\
    
R-FCN \cite{dai2016r}                       & 07+12   & ResNet-101   & 80.5 
    & 79.9 & 87.2 & 81.5 & 72.0 & 69.8 
    & 86.8 & 88.5 & 89.8 & 67.0 & 88.1 
    & 74.5 & 89.8 & 90.6 & 79.9 & 81.2 
    & 53.7 & 81.8 & 81.5 & 85.9 & 79.9 \\

\hline

{\bf SSD300*} \cite{liu2016ssd}             & 07+12   & VGGNet       & {\bf 77.2}         
    & 82.3 & 84.5 & 75.0 & 69.9 & 51.2
    & 85.2 & 85.6 & 87.5 & 63.0 & 82.6 
    & 76.2 & 84.2 & 86.5 & 83.8 & 78.6
    & 51.0 & 75.1 & 79.6 & 86.7 & 75.5 \\ 
    
SSD300 \cite{liu2016ssd}                    & 07+12   & VGGNet       & 77.5 
    & 79.5 & 83.9 & 76.0 & 69.6 & 50.5
    & 87.0 & 85.7 & 88.1 & 60.3 & 81.5 
    & 77.0 & 86.1 & 87.5 & 83.9 & 79.4 
    & 52.3 & 77.9 & 79.5 & 87.6 & 76.8 \\
    
DSSD321 \cite{fu2017dssd}                  & 07+12   & ResNet-101   & 78.6 
    & 81.9 & 84.9 & 80.5 & 68.4 & 53.9
    & 85.6 & 86.2 & 88.9 & 61.1 & 83.5 
    & 78.7 & 86.7 & 88.7 & 86.7 & 79.7 
    & 51.7 & 78.0 & 80.9 & 87.2 & 79.4 \\

\hline

{\bf StairNet}      & 07+12   & VGGNet       & {\bf 78.8}     
    & 81.3 & 85.4 & 77.8 & 72.1 & 59.2
    & 86.4 & 86.8 & 87.5 & 62.7 & 85.7
    & 76.0 & 84.1 & 88.4 & 86.1 & 78.8
    & 54.8 & 77.4 & 79.0 & 88.3 & 79.2 \\
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
\end{tablenotes}
\caption{{\bf PASCAL VOC 2007 \textit{test} detection results.} {\bf 07+12}: 07 trainval + 12 trainval. {\bf 07+12+S}: 07+12 plus segmentation labels.}   
\label{table:voc07}
\end{table*} 



%%% Table 2, results on VOC 2012
\begin{table*}
\resizebox{\textwidth}{!}{\begin{tabular}{c| c| c| c | c c c c c c c c c c c c c c c c c c c c c }
\hline
Method & data & network & mAP & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & horse & mbike & persn & plant & sheep & sofa & train & tv\\ 
\hline
HyperNet \cite{kong2016hypernet}            & 07++12    & VGGNet       & 71.4 
    & 84.2 & 78.5 & 73.6 & 55.6 & 53.7
    & 78.7 & 79.8 & 87.7 & 49.6 & 74.9
    & 52.1 & 86.0 & 81.7 & 83.3 & 81.8
    & 48.6 & 73.5 & 59.4 & 79.9 & 65.7 \\
Fr R-CNN \cite{ren2015faster}           & 07++12    & ResNet-101   & 73.8 
    & 86.5 & 81.6 & 77.2 & 58.0 & 51.0
    & 78.6 & 76.6 & 93.2 & 48.6 & 80.4
    & 59.0 & 92.1 & 85.3 & 84.8 & 80.7
    & 48.1 & 77.3 & 66.5 & 84.7 & 65.6 \\
ION \cite{bell2016inside}                   & 07++12+S  & VGGNet       & 76.4     
    & 87.5 & 84.7 & 76.8 & 63.8 & 58.3
    & 82.6 & 79.0 & 90.9 & 57.8 & 82.0
    & 64.7 & 88.9 & 86.5 & 84.7 & 82.3
    & 51.4 & 78.2 & 69.2 & 85.2 & 73.5 \\
% R-FCNmulti-sc \cite{dai2016r}               & 07++12    & ResNet-101   & 77.6
RFCN m-sc \cite{dai2016r}               & 07++12    & ResNet-101   & 77.6 
    & 86.9 & 83.4 & 81.5 & 63.8 & 62.4
    & 81.6 & 81.1 & 93.1 & 58.0 & 83.8
    & 60.8 & 92.7 & 86.0 & 84.6 & 84.4
    & 59.0 & 80.8 & 68.6 & 86.1 & 72.9 \\
\hline
YOLOv2 \cite{redmon2017yolo9000}            & 07++12    & Darknet-19   & 73.4 
    & 86.3 & 82.0 & 74.8 & 59.2 & 51.8 
    & 79.8 & 76.5 & 90.6 & 52.1 & 78.2 
    & 58.5 & 89.3 & 82.5 & 83.4 & 81.3
    & 49.1 & 77.2 & 62.4 & 83.8 & 68.7 \\ 
{\bf SSD300*} \cite{liu2016ssd}             & 07++12    & VGGNet       & {\bf 74.8} 
    & 87.7 & 83.4 & 73.0 & 60.3 & 47.7 
    & 80.6 & 76.7 & 91.5 & 57.6 & 77.6
    & 63.6 & 89.0 & 84.9 & 84.8 & 81.8
    & 48.9 & 77.9 & 72.3 & 86.1 & 71.2 \\ 
SSD300 \cite{liu2016ssd}                    & 07++12    & VGGNet       & 75.8 
    & 88.1 & 82.9 & 74.4 & 61.9 & 47.6 
    & 82.7 & 78.8 & 91.5 & 58.1 & 80.0
    & 64.1 & 89.4 & 85.7 & 85.5 & 82.6
    & 50.2 & 79.8 & 73.6 & 86.6 & 72.1 \\
DSSD321 \cite{fu2017dssd}                   & 07++12    & ResNet-101   & 76.3 
    & 87.3 & 83.3 & 75.4 & 64.6 & 46.8
    & 82.7 & 76.5 & 92.9 & 59.4 & 78.3
    & 64.3 & 91.5 & 86.6 & 86.6 & 82.1
    & 53.3 & 79.6 & 75.7 & 85.2 & 73.9 \\
\hline
{\bf StairNet}      & 07++12    & VGGNet       & {\bf 76.4} 
    & 87.7 & 83.1 & 74.6 & 64.2 & 51.3
    & 83.6 & 78.0 & 92.0 & 58.9 & 81.8
    & 66.2 & 89.6 & 86.0 & 84.9 & 82.6
    & 50.9 & 80.5 & 71.8 & 86.2 & 73.5 \\
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
\end{tablenotes}
\caption{{\bf PASCAL VOC 2012 \textit{test} detection results.} {\bf 07++12}: 07 trainval + 07 test + 12 trainval. {\bf 07+12+S}: 07+12 plus segmentation labels. Result link of \textbf{StairNet} : \url{http://host.robots.ox.ac.uk:8080/anonymous/SPPVPF.html} } 
\label{table:voc12}
\end{table*} 


%%% Table 3, scale-aware improvement [Type 2]
\begin{table*}
\resizebox{\textwidth}{!}{\begin{tabular}{c| c| c | c c c c c c c c c c c c c c c c c c c c c }
\hline
Method & scale & mAP & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & horse & mbike & persn & plant & sheep & sofa & train & tv \\ 
\hline
% SSD300*
%     & small     & 41.7         
%         & 47.2 & 64.7 & 35.2 & 23.2 &  8.5    
%         & 45.7 & 49.6 & {\bf 67.2} & 20.0 & 47.6      
%         & 30.1 & 53.1 & 61.6 & 46.9 & 27.8    
%         &  7.3 & 44.5 & {\bf 62.0} & 63.3 & 28.3 \\
% {\bf StairNet}
%     & small     & {\bf 50.6}
%         & {\bf 57.5} & {\bf 71.6} & {\bf 51.4} & {\bf 34.5} & {\bf 21.8}
%         & {\bf 54.2} & {\bf 56.2} & 65.4       & {\bf 24.0} & {\bf 73.2}
%         & {\bf 31.6} & {\bf 60.4} & {\bf 73.3} & {\bf 54.1} & {\bf 36.7}
%         & {\bf 21.5} & {\bf 51.7} & 59.5       & {\bf 70.0} & {\bf 43.8} \\
% \hline
SSD300* \cite{liu2016ssd}
    & small     & 41.7         
        & 47.2 & 64.7 & 35.2 & 23.2 &  8.5    
        & 45.7 & 49.6 & 67.2 & 20.0 & 47.6      
        & 30.1 & 53.1 & 61.6 & 46.9 & 27.8    
        &  7.3 & 44.5 & 62.0 & 63.3 & 28.3 \\
{\bf StairNet}
    & small     & \textbf{50.6}
        & 57.5 & 71.6 & 51.4 & 34.5 & 21.8
        & 54.2 & 56.2 & 65.4 & 24.0 & 73.2
        & 31.6 & 60.4 & 73.3 & 54.1 & 36.7
        & 21.5 & 51.7 & 59.5 & 70.0 & 43.8 \\
\hline
SSD300* \cite{liu2016ssd}
    & medium    & 76.8
        & 79.9 & 81.6 & 75.6 & 65.0 & 44.4    
        & 88.0 & 86.5 & 87.3 & 66.2 & 83.5
        & 74.9 & 83.6 & 87.7 & 86.5 & 80.3    
        & 46.5 & 75.2 & 78.9 & 86.1 & 77.0 \\
{\bf StairNet}
    & medium    & {\bf 78.0}
        & 79.1 & 83.1 & 77.9 & 69.2 & 55.0    
        & 88.1 & 86.7 & 88.0 & 62.5 & 83.1
        & 78.0 & 83.1 & 89.3 & 88.5 & 79.1    
        & 49.7 & 74.5 & 79.4 & 87.7 & 78.5 \\
\hline
SSD300* \cite{liu2016ssd}
    & large     & {\bf 80.4}
        & 90.5 & 88.1 & 80.1 & 80.5 & 63.7    
        & 88.3 & 90.2 & 90.7 & 50.9 & 82.6
        & 84.9 & 84.8 & 87.8 & 90.1 & 85.5    
        & 57.7 & 82.1 & 62.4 & 88.3 & 78.8 \\
{\bf StairNet}
    & large     & 78.5
        & 90.4 & 89.3 & 85.8 & 76.2 & 63.5    
        & 92.0 & 89.4 & 88.4 & 47.2 & 81.8
        & 80.3 & 80.5 & 88.2 & 89.8 & 83.5    
        & 52.8 & 76.6 & 46.5 & 89.9 & 79.0 \\
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
\end{tablenotes}
\caption{ {\bf Scale-aware evaluation on PASCAL VOC 2007 \textit{test}.} Two methods are trained on VOC 07+12. VGGNet is used as backbone in both methods.} 
\label{table:scale}
\end{table*} 
%%% Table 4, state-of-the-art on VOC 2007
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline
    Method & data & network & mAP & fps & lib\\
\hline
    YOLO \cite{redmon2017yolo9000}          & 07+12     & GoogLeNet  & 63.4        & 45    & DarkNet\\
    YOLOV2\_352 \cite{redmon2017yolo9000}   & 07+12     & DarkNet-19 & 73.7        & 81    & DarkNet\\
    YOLOV2\_544 \cite{redmon2017yolo9000}   & 07+12     & DarkNet-19 & 78.6        & 40    & DarkNet\\
    \rowcolor{Gray}
    SSD300*\cite{liu2016ssd}                & 07+12     & VGGNet     & 77.2        & 42    & PyTorch\\
    \rowcolor{Gray}
    SSD300 \cite{liu2016ssd}                & 07+12     & VGGNet     & 77.5        & 62    & Caffe  \\
    DSSD321 \cite{fu2017dssd}               & 07+12     & ResNet-101 & 78.6        & 9.5   & Caffe  \\
    RSSD300 \cite{jisoo2017rssd}            & 07+12     & VGGNet     & 78.5        & 35.0  & Caffe  \\
    DiCSSD300\cite{xiang2017context}        & 07+12     & VGGNet     & 78.1        & 40.8  & Caffe \\
\hline
    {\bf StairNet}                          & 07+12     & VGGNet     & {\bf 78.8}  & 30    & PyTorch\\
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
\end{tablenotes}
\caption{{\bf PASCAL VOC 2007 \textit{test} detection results.} Is is worth to note that PyTorch implementation runs slower (62fps $\rightarrow$ 42fps) and shows lower performance (77.5$\rightarrow$77.2) than Caffe implementation for exactly same algorithm (Row 4 \& 5). In spite of this disadvantage, \textbf{StairNet} outperforms other state-of-the-art methods.} 
\label{table:sota_voc07}
\end{table} 

%% Tabel 6, mAP@0.7+ from R-SSD [BMVC'17]
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c| c |c c c c c c|c}
\hline
&&&&Recall&&&&\\
Method & data&0.5&0.6&0.7&0.8&0.9&1&mAP@0.7+  \\
\hline
    SSD300* \cite{liu2016ssd}    & 07+12 &91.9&87.9&79.7&65.6&34.4&0& 44.9  \\
    R-SSD300 \cite{jisoo2017rssd}& 07+12 &92.7&88.4&82.4&68.9&37.6&0& 47.2  \\
    \textbf{StairNet}            & 07+12 &\textbf{94.3}&\textbf{90.1}&\textbf{83.5}&\textbf{70.1}&\textbf{38.8}&0& \textbf{48.1}  \\
\hline
\end{tabular}}
\begin{tablenotes}
\scriptsize
\item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
\end{tablenotes}
% \bigskip
\smallskip
\caption{{\bf mAP at Recall$\ge$0.7} mean average precision over recall$\ge$0.7 suggested by \cite{jisoo2017rssd}. In most practical cases, it is more important to achieve high-precision at high-recall range rather than at low-recall range. Our \textbf{StairNet} outperforms SSD and R-SSD. }
\label{tab:map07}
% \label{table:ele_op}
\end{table} 

% \iffalse
% \subsubsection{Effectiveness of each components}
% We know investigate the each components in our final StiarNet model.
% \fi


%%% Figure
% Occlusion: 002250, 006085, 007589
% Small: 000252, 001275, 002484, 002685, 004218, 007644, 002676
% Trunc: 000038, 001416
\begin{figure}
\centering
\hspace{-3em}
\subfigure[SSD300*]{
\begin{tabular}{c}
\includegraphics[width=40mm]{figures/teaser_SSD.jpg} \\
\includegraphics[width=40mm]{figures/trunc_ssd/000038.jpg} \\
\includegraphics[width=40mm]{figures/small_ssd/000252.jpg} \\
\includegraphics[width=40mm]{figures/small_ssd/007644.jpg} \\
\includegraphics[width=40mm]{figures/small_ssd/001275.jpg} \\
\end{tabular}
}
\hspace{-2em}
\subfigure[StairNet300]{
\begin{tabular}{c}
\includegraphics[width=40mm]{figures/small_stair/001856.png} \\
\includegraphics[width=40mm]{figures/trunc_stair/000038.png} \\
\includegraphics[width=40mm]{figures/small_stair/000252.png} \\
\includegraphics[width=40mm]{figures/small_stair/007644.png} \\
\includegraphics[width=40mm]{figures/small_stair/001275.png} \\
\end{tabular}
}
% \begin{tablenotes}
% \scriptsize
% \item \hspace*{\fill} {\bf *}: reproduced in PyTorch framework.
% \end{tablenotes}
\hspace{-3em}
\caption{\textbf{Qualitative results on PASCAL VOC 2007}. Green boxes indicate that \textbf{StairNet} performs better than SSD in challenge scenarios.}
\label{fig:results}
\end{figure}
